Latin American HECAP Physics Briefing Book 2025

The first process for the Latin American Strategy Forum for Research Infrastructure for High Energy, Cosmology and Astroparticle Physics (LASF4RI-HECAP) came to a conclusion in October 2020, with a Physics Briefing Book (PBB) presented in (2104.06852). Here we present an updated PBB, the result of the first update of LASF4RI-HECAP. The update process began with a call for White Papers from the HECAP community. The submitted contributions were presented at the III LASF4RI for HECAP Symposium: Update of the Strategic Plan, held at ICTP-SAIFR in S\~ao Paulo in August 26-29, 2024, with the participation of the Preparatory Group, High Level Strategy Group, Funding Agencies and representatives of similar efforts from around the globe. This updated PBB was written by the Preparatory Group based mainly on 46 White Papers submitted by the community and is organized around seven working groups: Astronomy, Astrophysics and Astroparticle Physics; Cosmology; Dark Matter; Neutrinos; Electroweak and Strong Interactions, Higgs Physics, CP and Flavour Physics and BSM; Instrumentation and Computing; Advanced Training and Capacity Building. It is intended to provide the essential input for the creation of a long-term HECAP strategy in the region.

==> Makefile <==
SHELL=/bin/bash

# Define the main LaTeX file and chapters
MAIN = LASF4RI-HECAP-PBB-2025
CHAPTERS = intro/intro astro/astro cosmo/cosmo dm/dm neutrinos/neutrinos ew-bsm/ew-bsm adsc/adsc ap_wp Training/Training
BIBS =  adsc/adsc astro/astro cosmo/cosmo dm/dm ew-bsm/ew-bsm intro/intro neutrinos/neutrinos Training/Training



# Default target: compile the PDF
all: $(MAIN).pdf

# Rule to create the PDF
$(MAIN).pdf: $(MAIN).tex $(CHAPTERS:=.tex) $(BIBS:=.bib)
	pdflatex $(MAIN)
	@for bib in $(BIBS); do \
		bibtex $$bib; \
	done
	makeglossaries $(MAIN)
	pdflatex $(MAIN)
	pdflatex $(MAIN)

# Rule to clean intermediate files
clean:
	rm -f *.aux *.log *.bbl *.blg *.toc *.out $(MAIN).pdf
	@for chap in $(CHAPTERS); do \
		rm -f $$chap.aux $$chap.bbl $$chap.blg; \
	done

.PHONY: all clean


==> adsc/adsc.tex <==
This chapter provides a comprehensive update on the landscape of instrumentation and computing within the Latin American High Energy Physics, Cosmology, and Astroparticle Physics (HECAP) community, building upon the initial LASF4RI strategic plan from 2020. It draws directly from white papers submitted for the current update process and discussions held at the "III LASF4RI for HECAP Symposium" in August 2024.

The goal of this chapter is to detail significant advancements and ongoing efforts across several key areas. Overlap with other chapters of this Briefing Book is unavoidable.

\section{Instrumentation and Computing in Latin American HECAP} \label{sec:instrumentation-computing} 

This section provides an update on the landscape of instrumentation and computing within the Latin American High Energy Physics (HECAP) community since the initial LASF4RI strategy report. It draws on submitted white papers and discussions from the III LASF4RI for the HECAP Symposium in August 2024 and builds on the 2020 report.

\subsection{Growth and Diversification of Local Instrumentation Capabilities} \label{subsec:local-instrumentation} 

The region has seen a \textbf{growth and diversification of local instrumentation capabilities}  since the initial 2020 report, with an increasing presence and construction of new local facilities for instrument development, building, testing, and characterization. This showcases a broad diversity of experience and skills developed across different groups and institutions in Latin America.

For instance, Argentina is building an \textbf{electron beam laboratory}  that will be the first large-scale, open, and user-oriented facility dedicated to neutron science in Latin America, located at the Atomic Center in Buenos Aires. This laboratory is being built in conjunction with a new nuclear reactor, which is already 80\% finished, and includes five foreseen experiments, two of which will have their instrumentation built by the Atomic Commission.

In Brazil, the National Institute for Science and Technology (INCT Brasil-CERN) is actively pursuing an interest in the \textbf{electronics for various detectors} , including gaseous detectors (like RPC from CMS), semiconductor detectors (focusing on FPGA boards), and photonic conversion detectors (such as those for LHCb's tracker). The initiative also aims to \textbf{involve Brazilian industry}  in this sector. 
%noting that CERN claims 80\% of its equipment is built in Brazil.

Chile has demonstrated leadership in hardware contributions to international projects, particularly for the \textbf{Jiangmen Underground Neutrino Observatory (JUNO)} . Chilean institutions, specifically PUC (Pontificia Universidad Católica de Chile), SAPHIR, and UCI (University of California, Irvine), led the design and manufacture of High Voltage Splitters (HVS) and Underwater Boxes (UWBs) in partnership with colleagues from France and China. These hardware responsibilities have now been completed, with SAPHIR remaining active in analysis processes. Brazilian research has also contributed to the purification of liquid argon for neutrino experiments. Furthermore, Argentina is involved in the research and development of low-threshold detectors.

\subsection{Sustained Involvement in Major International Collaborations} \label{subsec:international-collaborations} 

Latin American groups remain integral to major international HECAP experiments, with ongoing contributions to detector upgrades, data acquisition systems (DAQ), and trigger systems.

\begin{itemize} 
    \item \textbf{LHC Experiments:} 
    \begin{itemize} 
        \item The \textbf{\gls{ALICE} Experiment} attracts significant Brazilian participation, with a focus on heavy-ion collisions. The experiment has completed its LS2 upgrade, enabling high-rate data collection (50 kHz for lead-lead collisions), necessitating upgrades to the tracking and particle identification systems. Brazilian groups are developing a common readout unit for the \gls{ALICE} FoCal detector, based on FPGA processors, aiming for a time resolution of 20 picoseconds. 
        The Brazilian Center for Research in Energy and Materials (CNPEM) has recently joined the ALICE 3 magnet project with involvement in design and construction. Other Latin American countries, including Peru, Cuba, and Mexico, also participate in ALICE.
        \item In the \textbf{\gls{ATLAS} Experiment}, five Brazilian institutions are involved, contributing to over 29 PhD theses on \gls{ATLAS} topics. Brazilian groups engage in physics analysis, software development for performance, trigger and reconstruction, tier-2 data processing, and instrumentation development for semiconductor sensors and electronics. They also participate in Phase 1 and 2 upgrade projects and detector operations. Chile played a crucial role in building some of the muon chambers for the \gls{ATLAS} new small wheel upgrade. Argentina collaborates with \gls{ATLAS} on the trigger system, specifically on hardware and firmware implementation of algorithms for electron and photon identification using neural networks, aiming to provide 23\% of the necessary modules for the global trigger system.
        \item The \textbf{\gls{CMS} Experiment}  includes two Ecuadorian institutes, officially since 2016, with participation in physics analysis (top, Higgs, exotic searches) and service work, particularly with the Braille subsystem for luminosity and beam safety. Ecuadorian engineers were sent to CERN to prepare the Braille subsystem for run 3 startup. Chile and Peru have also expressed interest in joining \gls{CMS} with an institute. Fermilab hosts the US \gls{CMS} collaboration, which is building components for the High-Luminosity LHC (HL-LHC) accelerator and detector upgrades and conducting R\&D for the Future Circular Collider (FCC).
        \item Brazilian institutions, comprising three institutes, are involved in the \textbf{\gls{LHCb} Experiment}  and plan to continue their participation until 2041. Honduras is also interested in joining LHCb.
    \end{itemize} 
    \item \textbf{Neutrino Physics:} 
    \begin{itemize} 
        \item Brazil has made a significant in-kind contribution of cryogenic equipment, including pure liquid argon circulation and purification systems, to the \textbf{Deep Underground Neutrino Experiment (DUNE)}. In addition, Brazil will be responsible for the photodetectors in DUNE with the ARAPUCA design. 
        \item For \textbf{JUNO}, Chile demonstrated leadership in the design and manufacture of High Voltage Splitters and Underwater Boxes. Although the Brazilian contribution to \gls{JUNO} is currently small (four full-time equivalents within a collaboration of 700), it is viewed as a step in the right direction toward increased involvement with Chinese partners.
        \item The \textbf{Coherent Neutrino-Nucleus Scattering Experiment (CONNIE)}  is predominantly a Brazilian collaboration, with 70\% of its members from Brazil, and 95\% of \gls{CONNIE} members are also part of Oscura. \gls{CONNIE} is considered competitive for dark matter detection within the broader Dark Sector. There is also expressed interest in the \textbf{Hyper-Kamiokande}  experiment.
    \end{itemize} 
    \item \textbf{Dark Matter and Dark Energy Searches:} 
    \begin{itemize} 
        \item The Brazilian community has detailed its efforts in searching for dark matter and dark sector signals, utilizing a complementary approach that includes colliders, direct, and indirect detection, as well as neutrino physics, cosmology, and astrophysics. This community has demonstrated remarkable growth and consolidation, actively participating in large-scale and long-term international collaborations. By July 2024, more than 1,000 published papers and theses with Brazilian affiliations on dark matter and dark sectors had been produced. The flagship experiments in the region for dark matter research are the Cherenkov Telescope Array Observatory (CTAO) and the planned Southern Wide-field Gamma-ray Observatory (SWGO), both of which show potential for dark matter indirect detection.
        \item The \textbf{Oscura experiment}  is projected to be the best direct detection experiment for Light Dark Matter masses, with plans to build parts of the detectors in Argentina and Brazil, marking a potential milestone in Dark Matter physics in the region.
        \item Mexico aims to create a control center to process real-time data detected by the LIGO, VIRGO, and KAGRA interferometers in the coming years. Latin American groups are also increasingly involved in experiments such as the \textbf{Dark Energy Spectroscopic Instrument (DESI)} and the \textbf{Vera Rubin Observatory's Legacy Survey of Space and Time (LSST)}.
    \end{itemize} 
    \item \textbf{Astroparticle Physics \& Cosmology:} 
    \begin{itemize} 
        \item Participation extends to the Cherenkov Telescope Array (CTAO), the planned Southern Wide-field Gamma-ray Observatory (SWGO) and the Latin American Giant Observatory (LAGO). There is also an expressed interest in developing the South American Gravitational-Wave Observatory (SAGO). Chile will host the \textbf{\gls{LLAMA} observatory} , the first in the Southern Hemisphere. Latin American researchers' participation in cosmology experiments, such as \gls{LSST} and DESI, has increased, and their expertise in gravitational wave (GW) physics has been consolidated, with more groups joining second-generation detectors and members working in research units for third-generation detectors.
    \end{itemize} 
    \item \textbf{Future Colliders:} 
    \begin{itemize} 
        \item The Brazilian Center for Research in Energy and Materials (CNPEM) in Campinas, São Paulo has signed in November 2025 a cooperation agreement with CERN (the European Organization for Nuclear Research) to be part of a feasibility study for the Future Circular Collider. 
        \item Brazilian groups have shown interest in joining collaborations for the \textbf{Electron-Ion Collider (EIC)}, which is already approved by the DOE. Discussions are also ongoing regarding participation in future circular colliders, such as the \textbf{FCC}. Argentina has also created a dual doctoral program in Engineering and Information Technology to develop edge-of-technology infrastructure for such projects.
    \end{itemize} 
\end{itemize} 

\subsection{Strategic Advancement in Scientific Computing and Data Infrastructure} \label{subsec:computing-data} 

The increasing data volumes from current and future experiments, particularly those from the High-Luminosity LHC, necessitate continued strategic advances in computing and data infrastructure. Key areas of focus include:
\begin{itemize} 
    \item The \textbf{development and implementation of advanced data handling and analysis techniques}.
    \item Progress in \textbf{cloud computing initiatives}, such as the model being developed by the Brazilian INCT-FNAe.
    \item The application of \textbf{Machine Learning (ML) and Artificial Intelligence (AI)}  for data analysis, fast simulations, detector development, and trigger systems. For example, the \gls{ATLAS} collaboration is using GPUs in trigger and offline processing and experimenting with different data flows to enhance physics reach. Argentina is involved in the hardware and firmware implementation of algorithms for the \gls{ATLAS} global trigger system, including electron and photon identification using neural networks, with the goal of providing 23\% of the required modules.
    \item The need for \textbf{robust and reliable data storage and management solutions}.
    \item The development of \textbf{software tools and CI/CD practices}  to support collaborative research.
\end{itemize} 
A dedicated review of scenarios and proposals under the umbrella of a "SC+IT Hub" is underway, showcasing the effective use of hybrid spaces that integrate industrial and academic resources. This includes the introduction of AI models (such as LLMs) into scientific production, and the use of dedicated computing resources, Infrastructure as Code (IaC), and cloud technologies to create labs integrated into classrooms and curricula. These efforts aim to build robust, scalable, and accessible frameworks that support scientific endeavors and capacity-building projects, enhancing the participation of Latin American researchers in the global scientific community.

\subsection{Emphasis on Training and Capacity Building} \label{subsec:training-capacity-building} 

A crucial emphasis is placed on \textbf{developing and retaining highly qualified human resources}  in HECAP. This includes efforts to equip research teams with essential skills in documentation, protocol development, and data management. Advanced training programs are developed to harness regional capacities and expertise across Latin American countries. The role of international collaborations and networks in facilitating knowledge transfer and skill development is also crucial. It is important to consider local conditions to build a critical mass of human resources that remain in the region for long-term project development. Below is a list of some activities, with some overlap with the following chapter in this PBB.

\begin{itemize} 
\item The \textbf{ICTP South American Institute for Fundamental Research} (ICTP-SAIFR), based in São Paulo, Brazil, has become the premier hub in Latin American for HECAP activities, with International Schools in Particle Physics and Cosmology organized in partnership with ICTP-Trieste and several topical workshops and programs. In addition, it has an extensive outreach program in both Portuguese and Spanish.
    \item The \textbf{CERN Schools of Physics}  (Europe, Asia, Latin America) are two-week, residential programs targeted at PhD or advanced Master's students, sponsored by CERN and CIEMAT from Spain. These schools foster scientific training and networking among students and teachers from across the region and beyond. Recent schools were held in Mexico, Argentina, and Chile, while the 2025 edition took place in Costa Rica.
    \item The \textbf{CERN Summer Student Program} offers two- to three-month internships at CERN, with about half of participants coming from non-member states, making it highly accessible, though funding must be secured externally. CERN also organizes accelerator schools and computing schools; Chile is set to host a CERN Computing School in 2026.
     \item \textbf{The IDPASC Network} 
    The International Doctorate in Particle, Astrophysics and Cosmology has been running for over a decade, promoting international schools and visiting programs. Some institutions in Brazil, such as CBPF and UNESP, have been part of the IDPASC network for many years. Recently, UFRN and UFBA in Brazil and SAPHIR (Millennium Institute for Subatomic Physics at the High-Energy Frontier) in Chile also joined the network. As a result of this Latin American involvement in the network, the IDPASC school will be held in Latin America for the first time, at the International Institute of Physics in Natal, Brazil. The school will precede the ICHEP 2026 conference.
    
    \item \textbf{LA-CoNGA Physics}  is an open science education collaboration between Latin America and Europe for High Energy Physics. Associated hackathons, such as Cafina, are self-sustaining events that attract around 120 applicants annually, provide thousands of US dollars in prizes, and offer support to improve accessibility to internet or personal care during the event. Many participants return as hackers or even challengers in subsequent editions.
    \item ICTP \textbf{Physics Without Frontiers}  is a program that targets undergraduates, conducting "road trips" to deliver master classes in various countries, including Colombia, Ecuador, and Venezuela.
    \item In \textbf{Chile}, PhD scholarships are open to foreigners, with many recipients from Latin America (128 foreign students selected for the April-March academic year). Postdoctoral positions are also available for foreigners, including a special program with the Chinese Academy of Sciences in astronomy.
    \item \textbf{Ecuador} currently lacks universities that grant PhDs in physics, but Master's programs are beginning to emerge as a significant step forward. Over the past decade, Ecuador has expanded its HECAP research efforts by participating in international collaborations, including CMS, CTA, and LAGO.
    \item \textbf{Venezuela's}  efforts focus on access to education and capacity building, utilizing online platforms for events to build community and collaborations.
    \item The \textbf{Colombian scientific community} continues to make a strong contribution to theoretical high-energy physics, strengthening connections through workshops and meetings held over the last decade.
    \item In \textbf{Argentina}, a double doctoral program in engineering and information technology was created in 2020 with current participation of six ongoing students and one graduate.
    \item There is a recognized need to push initiatives for \textbf{collective applications for funding} , such as forming networks between CONACYT in Mexico, and relevant agencies in Argentina and Brazil, to organize workshops and invite students. The idea is to invite senior physicists for year-long sabbaticals to teach and train people in the region.
\end{itemize} 

\subsection{Fostering Collaboration and Networking} \label{subsec:collaboration-networking} 

The chapter highlights the crucial roles of collaborative efforts, knowledge sharing, and networks and consortia in boosting local efforts. This includes fostering both regional collaborations within Latin America and stronger ties with international partners.

\begin{itemize} 
    \item The \textbf{Latin American Association for High Energy, Cosmology and Astroparticle Physics (LAA-HECAP)} , established in November 2021 and hosted by ICTP-SAIFR, plays a significant role in fostering collaborations within the region. It currently has over 560 members and actively engages with ministries and funding agencies to promote strategic planning.
    \item The LASF4RI process itself has significantly enhanced the \textbf{visibility of the Latin American HECAP community} , as exemplified by a Symmetry Magazine diagram that summarized the Physics Briefing Book's findings.
    \item The \textbf{Colombian Network on High Energy Physics}  emphasizes synergistic efforts in dark matter, cosmology, astroparticle, and neutrino physics, demonstrating the increased interest and capabilities of Colombian researchers.
    \item \textbf{Mexico} is working to consolidate a network of researchers focused on Dirac materials, bridging condensed-matter physics and high-energy physics, and to foster collaborations throughout Latin America.
    \item The Brazilian \textbf{INCT Brasil-CERN} serves as a network of people and institutions with common goals, affiliated with the Ministry of Science and Technology. It aims to promote new transversal collaborations within the community and synergistic interactions with industry.
    \item Latin American groups involved in \textbf{gravitational wave science}  have increased their participation in second-generation detectors and have members in the consortia for third-generation detectors.
\end{itemize} 

\subsection{Addressing Challenges and Future Directions} \label{subsec:challenges-future} 

The Latin American HECAP community faces several challenges, including securing stable funding, ensuring access to shared infrastructures and tools, and addressing the training, recognition, and retention of human resources.

\begin{itemize} 
    \item \textbf{Financial constraints and funding instability}  are persistent issues across the region, making it difficult to find dedicated funding for upgrades and projects. Ecuador, for instance, explicitly highlights financial constraints and funding instability as major challenges.
    \item \textbf{Brain drain}  is a significant concern, with about 40\% of CERN users with Latin American nationality working elsewhere.
    \item \textbf{Mexico's CONACYT} has shifted its funding mechanisms to focus on the "human right of science".
    \item The Brazilian \textbf{INCT Brasil-CERN} actively lobbies funding agencies to secure stable funding for Memoranda of Understanding (MOUs) for large international collaborations. Argentina's participation in the \gls{ATLAS} upgrade, for example, relies on continued funding despite political changes impacting scientific ministries.
    \item \textbf{Chile's National Agency for Research and Development (ANID)}  system emphasizes the importance of political support for securing funding.
    \item For future projects, there is a recognized need for a \textbf{light-touch regional board}  drawn from existing bodies like LAA-HECAP and CLAF, to oversee a rotating calendar, select host sites, and appoint evaluation committees, ensuring accountability through transparent statutes and annual public reports.
    \item Initial \textbf{seed funding} for new initiatives could come from diverse sources, including UNESCO’s Participation Programme, OAS academic mobility funds, ERASMUS+ Capacity Building, and private foundations such as ICTP, Simons, and Sloan.
    \item LAA-HECAP is actively working to engage with ministries and funding agencies to promote the roll-out and development of the strategic planning process, demonstrating a proactive approach to addressing funding challenges.
    \item \textbf{Future directions} for Latin American HECAP include potential involvement in flagship projects, such as the SWGO, \gls{FCC}, and EIC. The LASF4RI process aims to outline these directions and strategic priorities to guide regional development.
\end{itemize} 

\section{Conclusions} \label{sec:conclusions} 

The Latin American HECAP community has demonstrated \textbf{remarkable growth and diversification in its research efforts}  since the initial LASF4RI strategy, expanding its involvement in numerous prestigious international collaborations and local initiatives. This progress underscores Latin America's growing contributions and engagement in critical areas of scientific inquiry.

Key aspects of this development include:
\begin{itemize} 
    \item \textbf{Broad Participation in International Experiments:}  Latin American researchers are actively involved in major global experiments across various thematic areas, as detailed in the Physics Briefing Book. These include:
    \begin{itemize} 
        \item \textbf{LHC Experiments:}  Continued and expanded participation in the Large Hadron Collider (LHC) experiments at CERN, such as ALICE, ATLAS, CMS, and LHCb, with contributions to detector upgrades and data analysis. For example, Chile has played a significant role in building muon chambers for ATLAS's new small wheel, and Brazil contributed to the LSDPC chip. Brazil currently has five institutions involved in ATLAS, with over 29 PhD theses completed on \gls{ATLAS} topics. Similarly, the CMS experiment receives key contributions from Brazil (3 groups), Mexico (5 groups), Chile, Colombia and Ecuador (2 groups each). The Brazilian group at LHCb, comprising three institutes, plans to continue participating until 2041. Honduras is interested in joining LHCb and Peru is interested in joining \gls{CMS} as institutes. Other Latin American countries, such as Peru, Cuba, and Mexico, also participate in the \gls{ALICE} experiment.
        \item \textbf{Neutrino Physics:}  Strong involvement in neutrino experiments such as the Deep Underground Neutrino Experiment (DUNE), the Jiangmen Underground Neutrino Observatory (JUNO) in China, where Latin American groups, particularly from Chile, led the design and manufacture of High Voltage Splitters and Underwater Boxes, and the Coherent Neutrino-Nucleus Scattering Experiment (CONNIE). There is also expressed interest in Hyper-Kamiokande.
        \item \textbf{Dark Matter and Dark Energy Searches:}  Growing engagement in experiments like the Dark Energy Spectroscopic Instrument (DESI), the Vera Rubin Observatory's Legacy Survey of Space and Time (LSST), and various dark matter dedicated projects such as \gls{SWGO} and efforts related to CTA. The Brazilian dark matter research community has shown remarkable growth since 2011, with over 1000 published papers and theses by mid-2024. Mexico aims to create a control center to process real-time data detected by LIGO, VIRGO, and KAGRA interferometers in the coming years.
        \item \textbf{Astroparticle Physics \& Cosmology:}  Participation in the Cherenkov Telescope Array (CTA), the Latin American Giant Observatory (LAGO), and gravitational wave science, with an expressed interest in developing the South American Gravitational-Wave Observatory (SAGO). Chile will host the \gls{LLAMA} observatory, the first in the Southern Hemisphere.
        \item \textbf{Future Colliders:}  Brazilian groups are interested in joining collaborations for the Electron-Ion Collider (EIC), which is already approved by the DOE. Discussions are also ongoing regarding participation in future circular colliders, such as the FCC.
    \end{itemize} 
    \item \textbf{Instrumentation and Computing Advancements:}  The region has seen a \textbf{growth and diversification of local instrumentation capabilities}, moving towards the construction of new local facilities for instrument development and testing. There's a strong focus on strategic advancements in scientific computing and data infrastructure, including:
    \begin{itemize} 
        \item Development and implementation of \textbf{advanced data handling and analysis techniques}.
        \item Progress in \textbf{cloud computing initiatives}, such as the model by the Brazilian INCT-FNAe.
        \item Application of \textbf{Machine Learning (ML) and Artificial Intelligence (AI)}  for data analysis, fast simulations, detector development, and trigger systems. For example, the \gls{ATLAS} collaboration uses GPUs for trigger and offline processing and is exploring different data flows to enhance physics reach. Argentina is involved in the hardware and firmware implementation of algorithms for the \gls{ATLAS} global trigger system, including electron and photon identification using neural networks, with the aim of providing 23\% of the required modules.
        \item Initiatives to develop \textbf{software tools and CI/CD practices} .
    \end{itemize} 
    \item \textbf{Capacity Building and Training:}  A crucial emphasis is placed on \textbf{developing and retaining highly qualified human resources}  in HECAP. This includes:
    \begin{itemize} 
        \item The \textbf{CERN Schools of Physics}  (Europe, Asia, Latin America), which support Latin American students. The last three schools were held in Mexico, Argentina, and Chile, with the next school planned for Costa Rica in 2025. These are two-week, residential programs for PhD or advanced Master's students, sponsored by CERN and CIEMAT from Spain. CERN also organizes Accelerator and Computing schools, and Brazil is slated to host a Computing School in 2026.
        \item Programs like \textbf{LA-CoNGA Physics}, an open science education collaboration between Latin America and Europe for High Energy Physics, and associated hackathons (e.g., Coafina, which recently completed its third edition).
        \item \textbf{Mobility programs}  for students and professors between Latin American institutions and international labs like CERN and Fermilab. Fermilab's ``Physics Without Frontiers'' program targets undergraduates, and a proposed Mobility Initiative with LAA-HECAP aims to foster collaboration and career paths in neutrino research. Chile offers PhD scholarships open to foreign students, with many recipients from Latin America (128 foreign students selected for the April-March academic year). Ecuador currently lacks universities that grant PhDs in physics, but Master's programs are beginning to emerge as a significant step. Venezuela's efforts focus on access to education and capacity building, utilizing online platforms for events to build community.
    \end{itemize} 
    \item \textbf{Strengthening Collaboration and Funding Advocacy:}  The LASF4RI process itself has significantly fostered regional collaboration and knowledge sharing. There is a recognized need to \textbf{engage proactively with funding agencies and national authorities}  to secure stable and predictable funding for both regional projects and international participation. Challenges include financial constraints, funding instability, and personnel turnover. Brazil, as an associate member of CERN, highlights the need for dedicated funding for researchers' work and mobility, distinct from treaty contributions. Mexico's CONACYT, which is transitioning into the Ministry of Science, Humanities, Technologies, and Innovation, has fundamentally shifted its funding mechanisms to focus on the ``human right of science''. The Brazilian INCT Brasil-CERN actively lobbies funding agencies to secure stable funding for MOUs related to large collaborations. Argentina's participation in the \gls{ATLAS} upgrade relies on continued funding, despite political changes impacting scientific ministries.
\end{itemize} 

The progress made, as highlighted by the submitted white papers and discussions at the LASF4RI symposia, indicates Latin America's growing capacity to play a significant role in the global HECAP landscape, emphasizing both its regional strengths (e.g., geographical advantages for astroparticle observatories) and its increasing impact in international flagship projects.

%\bibliographystyle{plain} 
%\bibliography{adsc/adsc} 

